INTERPLAY: An Intelligent Model for Predicting Performance Degradation due to Multi-cache Way-disabling

Modern and future processors need to remain functionally correct in the presence of permanent faults to sustain scaling benefits and limit field returns. This paper presents a combined analytical and microarchitectural simulation-based framework called INTERPLAY, that can rapidly predict, at design-time, the performance degradation expected from a processor employing way-disabling to handle permanent faults in caches while in-the-field. The proposed model can predict a program's performance with an accuracy of up to 98.40% for a processor with a two-level cache hierarchy, when multiple caches suffer from faults and need to disable one or more of their ways. INTERPLAY is 9.2x faster than an exhaustive simulation approach since it only needs the training simulation runs for the single-cache way-disabling configurations to predict the performance for any multi-cache way-disabling configuration.

==> Background.tex <==
\section{Problem Formulation}
\vspace{0.5cm}
\subsection{Persistent Errors and Cache Disabling}
Persistent errors and cause of them
 The cache disabling due to power issues and reliability issues. However in this work we will focus on the cache disabling due to reliability reasons.
 Some other works operate at very low voltage in order to improve cache lifetime
\subsection{Naive Exhaustive-Based Simulation Solution}
One way to determine the performance degradation due to cache disabling is to simulate the program for each possible FMP. For each FMP this will require p simulations one for each FM. Then the probability and performance of an FMP is obtained as per Section 3. The performance distribution is produced by summing the probabilities of all FMP that lead to same performance.
though the naive method is exact it is in general nontractable because it simply requires too many simulations. For example for an 8 way set with 64B per block, for T=3 years and Dt=1 day, i.e. p=1095, this method will require to generate (1096) 4096 FMPs and for each FMP to perform 1095 simulations!

\subsection{Performance Predictability Models}
Several works try to predict the performance degradation due to cache disabling.
Some of these works. The work in [Damien] proposes a firs order model however this work assumes high probability of failure that does not lead to all the combinations.

==> applicability.tex <==
\section{Model Applicability} \label{applicability}

Additionally, the model can be used in real time to reduce the number of field returns by providing an online performance analysis and exploring the trade-off with the cost of replacement. 
Another real time applicability of the model it is to use it for reducing leakage power by turning off some parts of the cache. This work will be used on top of disabling techniques to consider the trade-off between power and performance. 
